Conformal Data for the O(3) Wilson-Fisher Conformal Field Theory from Fuzzy Sphere Realization of the Quantum Rotor Model

We present a model for strongly interacting fermions with internal O(3) symmetry on the fuzzy-sphere that (i) preserves the rotational symmetry of the fuzzy sphere and (ii) undergoes a quantum phase transition in the (2+1)-dimensional O(3) Wilson-Fisher universality class. Using exact diagonalization (ED) and density matrix renormalization group (DMRG), we locate the quantum critical point via conformal perturbation theory and obtain scaling dimensions from finite-size spectra. We identify 24 primary operators and determine some of their operator product expansion coefficients through first-order conformal perturbation theory. The results are benchmarked against conformal bootstrap and large quantum-number expansions and reveal a weakly irrelevant operator that plays a role in dimerized antiferromagnets. Our work establishes the fuzzy sphere as a general framework for quantitatively accessing conformal data in non-Abelian conformal field theories (CFTs).

==> Delta_Tables/Delta_S6_-_L0.tex <==
\begin{tabular}{|p{2cm}|p{1.5cm}|p{4.9cm}||p{2cm}|p{1.5cm}|p{4.9cm}|}
\hline
Index & Method & $\Delta$ & Index & Method & $\Delta$ \\
\hline
1 & ED & $8.8069$ $(10)$, $8.8056$ $(9)$ & 2 & ED & $10.1560$ $(10)$, $10.1037$ $(9)$ \\
\hline
\end{tabular}

==> Delta_Tables/Delta_S7_+_L0.tex <==
\begin{tabular}{|p{2cm}|p{1.5cm}|p{4.9cm}||p{2cm}|p{1.5cm}|p{4.9cm}|}
\hline
Index & Method & $\Delta$ & Index & Method & $\Delta$ \\
\hline
1 & ED & $10.3983$ $(10)$ & & & \\
\hline
\end{tabular}

==> Delta_Tables/Delta_S7_+_L1.tex <==
\begin{tabular}{|p{2cm}|p{1.5cm}|p{4.9cm}||p{2cm}|p{1.5cm}|p{4.9cm}|}
\hline
Index & Method & $\Delta$ & Index & Method & $\Delta$ \\
\hline
1 & ED & $9.3458$ $(10)$ & 3 & ED & $10.7255$ $(10)$ \\
\hline
1 & DMRG & $9.1532$ $(20)$, $9.2270$ $(16)$ & 4 & ED & $11.1102$ $(10)$ \\
\hline
2 & ED & $10.2818$ $(10)$ & 5 & ED & $11.1805$ $(10)$ \\
\hline
\end{tabular}

==> Delta_Tables/Delta_S7_+_L2.tex <==
\begin{tabular}{|p{2cm}|p{1.5cm}|p{4.9cm}||p{2cm}|p{1.5cm}|p{4.9cm}|}
\hline
Index & Method & $\Delta$ & Index & Method & $\Delta$ \\
\hline
1 & ED & $9.6012$ $(10)$ & 4 & ED & $10.8940$ $(10)$ \\
\hline
2 & ED & $10.0748$ $(10)$ & 5 & ED & $10.9786$ $(10)$ \\
\hline
3 & ED & $10.4556$ $(10)$ & & & \\
\hline
\end{tabular}

==> Delta_Tables/Delta_S7_+_L3.tex <==
\begin{tabular}{|p{2cm}|p{1.5cm}|p{4.9cm}||p{2cm}|p{1.5cm}|p{4.9cm}|}
\hline
Index & Method & $\Delta$ & Index & Method & $\Delta$ \\
\hline
1 & ED & $9.8639$ $(10)$ & 4 & ED & $10.6808$ $(10)$ \\
\hline
2 & ED & $10.2074$ $(10)$ & 5 & ED & $10.9424$ $(10)$ \\
\hline
3 & ED & $10.5616$ $(10)$ & 6 & ED & $11.1448$ $(10)$ \\
\hline
\end{tabular}

==> Delta_Tables/Delta_S7_+_L4.tex <==
\begin{tabular}{|p{2cm}|p{1.5cm}|p{4.9cm}||p{2cm}|p{1.5cm}|p{4.9cm}|}
\hline
Index & Method & $\Delta$ & Index & Method & $\Delta$ \\
\hline
1 & ED & $10.0686$ $(10)$ & 4 & ED & $10.8779$ $(10)$ \\
\hline
2 & ED & $10.3459$ $(10)$ & 5 & ED & $11.0600$ $(10)$ \\
\hline
3 & ED & $10.5834$ $(10)$ & & & \\
\hline
\end{tabular}

==> Delta_Tables/Delta_S7_-_L0.tex <==
\begin{tabular}{|p{2cm}|p{1.5cm}|p{4.9cm}||p{2cm}|p{1.5cm}|p{4.9cm}|}
\hline
Index & Method & $\Delta$ & Index & Method & $\Delta$ \\
\hline
1 & ED & $7.4991$ $(10)$ & 2 & ED & $9.5674$ $(10)$ \\
\hline
1 & DMRG & $7.2265$ $(20)$, $7.3220$ $(16)$ & 3 & ED & $11.1251$ $(10)$ \\
\hline
\end{tabular}

==> Delta_Tables/Delta_S7_-_L1.tex <==
\begin{tabular}{|p{2cm}|p{1.5cm}|p{4.9cm}||p{2cm}|p{1.5cm}|p{4.9cm}|}
\hline
Index & Method & $\Delta$ & Index & Method & $\Delta$ \\
\hline
1 & ED & $8.4354$ $(10)$ & 3 & ED & $10.7230$ $(10)$ \\
\hline
2 & ED & $10.3625$ $(10)$ & & & \\
\hline
\end{tabular}

==> Delta_Tables/Delta_S7_-_L2.tex <==
\begin{tabular}{|p{2cm}|p{1.5cm}|p{4.9cm}||p{2cm}|p{1.5cm}|p{4.9cm}|}
\hline
Index & Method & $\Delta$ & Index & Method & $\Delta$ \\
\hline
1 & ED & $9.1508$ $(10)$ & 3 & ED & $10.2780$ $(10)$ \\
\hline
2 & ED & $9.4721$ $(10)$ & 4 & ED & $10.9884$ $(10)$ \\
\hline
\end{tabular}

==> Delta_Tables/Delta_S7_-_L3.tex <==
\begin{tabular}{|p{2cm}|p{1.5cm}|p{4.9cm}||p{2cm}|p{1.5cm}|p{4.9cm}|}
\hline
Index & Method & $\Delta$ & Index & Method & $\Delta$ \\
\hline
1 & ED & $9.6538$ $(10)$ & 4 & ED & $10.7293$ $(10)$ \\
\hline
2 & ED & $10.1238$ $(10)$ & 5 & ED & $11.1397$ $(10)$ \\
\hline
3 & ED & $10.3304$ $(10)$ & & & \\
\hline
\end{tabular}

==> Delta_Tables/Delta_S7_-_L4.tex <==
\begin{tabular}{|p{2cm}|p{1.5cm}|p{4.9cm}||p{2cm}|p{1.5cm}|p{4.9cm}|}
\hline
Index & Method & $\Delta$ & Index & Method & $\Delta$ \\
\hline
1 & ED & $10.5577$ $(10)$ & 3 & ED & $10.9116$ $(10)$ \\
\hline
2 & ED & $10.6866$ $(10)$ & & & \\
\hline
\end{tabular}

==> Delta_Tables/all_delta_tables.tex <==
% ===== S = 0, parity + =====
\begin{table}[htbp]
\centering
\caption{Scaling dimension for the sector $S=0^{+}, L=0$. For the ED and DMRG data, the numbers in bracket is the corresponding system size. For the $\epsilon$-expansion and large-$N$ expansion, the numbers in the bracket indicate the order of the expansion.}}
\input{Delta_Tables/Delta_S0_+_L0.tex}
\end{table}
\begin{table}[htbp]
\centering
\caption{Scaling dimension for the sector $S=0^{+}, L=1$. For the ED and DMRG data, the numbers in bracket is the corresponding system size. For the $\epsilon$-expansion and large-$N$ expansion, the numbers in the bracket indicate the order of the expansion.}}
\input{Delta_Tables/Delta_S0_+_L1.tex}
\end{table}
\begin{table}[htbp]
\centering
\caption{Scaling dimension for the sector $S=0^{+}, L=2$. For the ED and DMRG data, the numbers in bracket is the corresponding system size. For the $\epsilon$-expansion and large-$N$ expansion, the numbers in the bracket indicate the order of the expansion.}}
\input{Delta_Tables/Delta_S0_+_L2.tex}
\end{table}
\begin{table}[htbp]
\centering
\caption{Scaling dimension for the sector $S=0^{+}, L=3$. For the ED and DMRG data, the numbers in bracket is the corresponding system size. For the $\epsilon$-expansion and large-$N$ expansion, the numbers in the bracket indicate the order of the expansion.}}
\input{Delta_Tables/Delta_S0_+_L3.tex}
\end{table}
\begin{table}[htbp]
\centering
\caption{Scaling dimension for the sector $S=0^{+}, L=4$. For the ED and DMRG data, the numbers in bracket is the corresponding system size. For the $\epsilon$-expansion and large-$N$ expansion, the numbers in the bracket indicate the order of the expansion.}}
\input{Delta_Tables/Delta_S0_+_L4.tex}
\end{table}
\begin{table}[htbp]
\centering
\caption{Scaling dimension for the sector $S=0^{+}, L=5$. For the ED and DMRG data, the numbers in bracket is the corresponding system size. For the $\epsilon$-expansion and large-$N$ expansion, the numbers in the bracket indicate the order of the expansion.}}
\input{Delta_Tables/Delta_S0_+_L5.tex}
\end{table}
\begin{table}[htbp]
\centering
\caption{Scaling dimension for the sector $S=0^{+}, L=6$. For the ED and DMRG data, the numbers in bracket is the corresponding system size. For the $\epsilon$-expansion and large-$N$ expansion, the numbers in the bracket indicate the order of the expansion.}}
\input{Delta_Tables/Delta_S0_+_L6.tex}
\end{table}
\begin{table}[htbp]
\centering
\caption{Scaling dimension for the sector $S=0^{+}, L=7$. For the ED and DMRG data, the numbers in bracket is the corresponding system size. For the $\epsilon$-expansion and large-$N$ expansion, the numbers in the bracket indicate the order of the expansion.}}
\input{Delta_Tables/Delta_S0_+_L7.tex}
\end{table}

% ===== S = 0, parity - =====
\begin{table}[htbp]
\centering
\caption{Scaling dimension for the sector $S=0^{-}, L=0$. For the ED and DMRG data, the numbers in bracket is the corresponding system size. For the $\epsilon$-expansion and large-$N$ expansion, the numbers in the bracket indicate the order of the expansion.}}
\input{Delta_Tables/Delta_S0_-_L0.tex}
\end{table}
\begin{table}[htbp]
\centering
\caption{Scaling dimension for the sector $S=0^{-}, L=1$. For the ED and DMRG data, the numbers in bracket is the corresponding system size. For the $\epsilon$-expansion and large-$N$ expansion, the numbers in the bracket indicate the order of the expansion.}}
\input{Delta_Tables/Delta_S0_-_L1.tex}
\end{table}
\begin{table}[htbp]
\centering
\caption{Scaling dimension for the sector $S=0^{-}, L=2$. For the ED and DMRG data, the numbers in bracket is the corresponding system size. For the $\epsilon$-expansion and large-$N$ expansion, the numbers in the bracket indicate the order of the expansion.}}
\input{Delta_Tables/Delta_S0_-_L2.tex}
\end{table}
\begin{table}[htbp]
\centering
\caption{Scaling dimension for the sector $S=0^{-}, L=3$. For the ED and DMRG data, the numbers in bracket is the corresponding system size. For the $\epsilon$-expansion and large-$N$ expansion, the numbers in the bracket indicate the order of the expansion.}}
\input{Delta_Tables/Delta_S0_-_L3.tex}
\end{table}
\begin{table}[htbp]
\centering
\caption{Scaling dimension for the sector $S=0^{-}, L=4$. For the ED and DMRG data, the numbers in bracket is the corresponding system size. For the $\epsilon$-expansion and large-$N$ expansion, the numbers in the bracket indicate the order of the expansion.}}
\input{Delta_Tables/Delta_S0_-_L4.tex}
\end{table}
\begin{table}[htbp]
\centering
\caption{Scaling dimension for the sector $S=0^{-}, L=5$. For the ED and DMRG data, the numbers in bracket is the corresponding system size. For the $\epsilon$-expansion and large-$N$ expansion, the numbers in the bracket indicate the order of the expansion.}}
\input{Delta_Tables/Delta_S0_-_L5.tex}
\end{table}
\begin{table}[htbp]
\centering
\caption{Scaling dimension for the sector $S=0^{-}, L=6$. For the ED and DMRG data, the numbers in bracket is the corresponding system size. For the $\epsilon$-expansion and large-$N$ expansion, the numbers in the bracket indicate the order of the expansion.}}
\input{Delta_Tables/Delta_S0_-_L6.tex}
\end{table}
\begin{table}[htbp]
\centering
\caption{Scaling dimension for the sector $S=0^{-}, L=7$. For the ED and DMRG data, the numbers in bracket is the corresponding system size. For the $\epsilon$-expansion and large-$N$ expansion, the numbers in the bracket indicate the order of the expansion.}}
\input{Delta_Tables/Delta_S0_-_L7.tex}
\end{table}

% ===== S = 1, parity + =====
\begin{table}[htbp]
\centering
\caption{Scaling dimension for the sector $S=1^{+}, L=0$. For the ED and DMRG data, the numbers in bracket is the corresponding system size. For the $\epsilon$-expansion and large-$N$ expansion, the numbers in the bracket indicate the order of the expansion.}}
\input{Delta_Tables/Delta_S1_+_L0.tex}
\end{table}
\begin{table}[htbp]
\centering
\caption{Scaling dimension for the sector $S=1^{+}, L=1$. For the ED and DMRG data, the numbers in bracket is the corresponding system size. For the $\epsilon$-expansion and large-$N$ expansion, the numbers in the bracket indicate the order of the expansion.}}
\input{Delta_Tables/Delta_S1_+_L1.tex}
\end{table}
\begin{table}[htbp]
\centering
\caption{Scaling dimension for the sector $S=1^{+}, L=2$. For the ED and DMRG data, the numbers in bracket is the corresponding system size. For the $\epsilon$-expansion and large-$N$ expansion, the numbers in the bracket indicate the order of the expansion.}}
\input{Delta_Tables/Delta_S1_+_L2.tex}
\end{table}
\begin{table}[htbp]
\centering
\caption{Scaling dimension for the sector $S=1^{+}, L=3$. For the ED and DMRG data, the numbers in bracket is the corresponding system size. For the $\epsilon$-expansion and large-$N$ expansion, the numbers in the bracket indicate the order of the expansion.}}
\input{Delta_Tables/Delta_S1_+_L3.tex}
\end{table}
\begin{table}[htbp]
\centering
\caption{Scaling dimension for the sector $S=1^{+}, L=4$. For the ED and DMRG data, the numbers in bracket is the corresponding system size. For the $\epsilon$-expansion and large-$N$ expansion, the numbers in the bracket indicate the order of the expansion.}}
\input{Delta_Tables/Delta_S1_+_L4.tex}
\end{table}
\begin{table}[htbp]
\centering
\caption{Scaling dimension for the sector $S=1^{+}, L=5$. For the ED and DMRG data, the numbers in bracket is the corresponding system size. For the $\epsilon$-expansion and large-$N$ expansion, the numbers in the bracket indicate the order of the expansion.}}
\input{Delta_Tables/Delta_S1_+_L5.tex}
\end{table}
\begin{table}[htbp]
\centering
\caption{Scaling dimension for the sector $S=1^{+}, L=6$. For the ED and DMRG data, the numbers in bracket is the corresponding system size. For the $\epsilon$-expansion and large-$N$ expansion, the numbers in the bracket indicate the order of the expansion.}}
\input{Delta_Tables/Delta_S1_+_L6.tex}
\end{table}
\begin{table}[htbp]
\centering
\caption{Scaling dimension for the sector $S=1^{+}, L=7$. For the ED and DMRG data, the numbers in bracket is the corresponding system size. For the $\epsilon$-expansion and large-$N$ expansion, the numbers in the bracket indicate the order of the expansion.}}
\input{Delta_Tables/Delta_S1_+_L7.tex}
\end{table}

% ===== S = 1, parity - =====
\begin{table}[htbp]
\centering
\caption{Scaling dimension for the sector $S=1^{-}, L=0$. For the ED and DMRG data, the numbers in bracket is the corresponding system size. For the $\epsilon$-expansion and large-$N$ expansion, the numbers in the bracket indicate the order of the expansion.}}
\input{Delta_Tables/Delta_S1_-_L0.tex}
\end{table}
\begin{table}[htbp]
\centering
\caption{Scaling dimension for the sector $S=1^{-}, L=1$. For the ED and DMRG data, the numbers in bracket is the corresponding system size. For the $\epsilon$-expansion and large-$N$ expansion, the numbers in the bracket indicate the order of the expansion.}}
\input{Delta_Tables/Delta_S1_-_L1.tex}
\end{table}
\begin{table}[htbp]
\centering
\caption{Scaling dimension for the sector $S=1^{-}, L=2$. For the ED and DMRG data, the numbers in bracket is the corresponding system size. For the $\epsilon$-expansion and large-$N$ expansion, the numbers in the bracket indicate the order of the expansion.}}
\input{Delta_Tables/Delta_S1_-_L2.tex}
\end{table}
\begin{table}[htbp]
\centering
\caption{Scaling dimension for the sector $S=1^{-}, L=3$. For the ED and DMRG data, the numbers in bracket is the corresponding system size. For the $\epsilon$-expansion and large-$N$ expansion, the numbers in the bracket indicate the order of the expansion.}}
\input{Delta_Tables/Delta_S1_-_L3.tex}
\end{table}
\begin{table}[htbp]
\centering
\caption{Scaling dimension for the sector $S=1^{-}, L=4$. For the ED and DMRG data, the numbers in bracket is the corresponding system size. For the $\epsilon$-expansion and large-$N$ expansion, the numbers in the bracket indicate the order of the expansion.}}
\input{Delta_Tables/Delta_S1_-_L4.tex}
\end{table}
\begin{table}[htbp]
\centering
\caption{Scaling dimension for the sector $S=1^{-}, L=5$. For the ED and DMRG data, the numbers in bracket is the corresponding system size. For the $\epsilon$-expansion and large-$N$ expansion, the numbers in the bracket indicate the order of the expansion.}}
\input{Delta_Tables/Delta_S1_-_L5.tex}
\end{table}
\begin{table}[htbp]
\centering
\caption{Scaling dimension for the sector $S=1^{-}, L=6$. For the ED and DMRG data, the numbers in bracket is the corresponding system size. For the $\epsilon$-expansion and large-$N$ expansion, the numbers in the bracket indicate the order of the expansion.}}
\input{Delta_Tables/Delta_S1_-_L6.tex}
\end{table}
\begin{table}[htbp]
\centering
\caption{Scaling dimension for the sector $S=1^{-}, L=7$. For the ED and DMRG data, the numbers in bracket is the corresponding system size. For the $\epsilon$-expansion and large-$N$ expansion, the numbers in the bracket indicate the order of the expansion.}}
\input{Delta_Tables/Delta_S1_-_L7.tex}
\end{table}

% ===== S = 2, parity + =====
\begin{table}[htbp]
\centering
\caption{Scaling dimension for the sector $S=2^{+}, L=0$. For the ED and DMRG data, the numbers in bracket is the corresponding system size. For the $\epsilon$-expansion and large-$N$ expansion, the numbers in the bracket indicate the order of the expansion.}}
\input{Delta_Tables/Delta_S2_+_L0.tex}
\end{table}
\begin{table}[htbp]
\centering
\caption{Scaling dimension for the sector $S=2^{+}, L=1$. For the ED and DMRG data, the numbers in bracket is the corresponding system size. For the $\epsilon$-expansion and large-$N$ expansion, the numbers in the bracket indicate the order of the expansion.}}
\input{Delta_Tables/Delta_S2_+_L1.tex}
\end{table}
\begin{table}[htbp]
\centering
\caption{Scaling dimension for the sector $S=2^{+}, L=2$. For the ED and DMRG data, the numbers in bracket is the corresponding system size. For the $\epsilon$-expansion and large-$N$ expansion, the numbers in the bracket indicate the order of the expansion.}}
\input{Delta_Tables/Delta_S2_+_L2.tex}
\end{table}
\begin{table}[htbp]
\centering
\caption{Scaling dimension for the sector $S=2^{+}, L=3$. For the ED and DMRG data, the numbers in bracket is the corresponding system size. For the $\epsilon$-expansion and large-$N$ expansion, the numbers in the bracket indicate the order of the expansion.}}
\input{Delta_Tables/Delta_S2_+_L3.tex}
\end{table}
\begin{table}[htbp]
\centering
\caption{Scaling dimension for the sector $S=2^{+}, L=4$. For the ED and DMRG data, the numbers in bracket is the corresponding system size. For the $\epsilon$-expansion and large-$N$ expansion, the numbers in the bracket indicate the order of the expansion.}}
\input{Delta_Tables/Delta_S2_+_L4.tex}
\end{table}
\begin{table}[htbp]
\centering
\caption{Scaling dimension for the sector $S=2^{+}, L=5$. For the ED and DMRG data, the numbers in bracket is the corresponding system size. For the $\epsilon$-expansion and large-$N$ expansion, the numbers in the bracket indicate the order of the expansion.}}
\input{Delta_Tables/Delta_S2_+_L5.tex}
\end{table}
\begin{table}[htbp]
\centering
\caption{Scaling dimension for the sector $S=2^{+}, L=6$. For the ED and DMRG data, the numbers in bracket is the corresponding system size. For the $\epsilon$-expansion and large-$N$ expansion, the numbers in the bracket indicate the order of the expansion.}}
\input{Delta_Tables/Delta_S2_+_L6.tex}
\end{table}
\begin{table}[htbp]
\centering
\caption{Scaling dimension for the sector $S=2^{+}, L=7$. For the ED and DMRG data, the numbers in bracket is the corresponding system size. For the $\epsilon$-expansion and large-$N$ expansion, the numbers in the bracket indicate the order of the expansion.}}
\input{Delta_Tables/Delta_S2_+_L7.tex}
\end{table}

% ===== S = 2, parity - =====
\begin{table}[htbp]
\centering
\caption{Scaling dimension for the sector $S=2^{-}, L=0$. For the ED and DMRG data, the numbers in bracket is the corresponding system size. For the $\epsilon$-expansion and large-$N$ expansion, the numbers in the bracket indicate the order of the expansion.}}
\input{Delta_Tables/Delta_S2_-_L0.tex}
\end{table}
\begin{table}[htbp]
\centering
\caption{Scaling dimension for the sector $S=2^{-}, L=1$. For the ED and DMRG data, the numbers in bracket is the corresponding system size. For the $\epsilon$-expansion and large-$N$ expansion, the numbers in the bracket indicate the order of the expansion.}}
\input{Delta_Tables/Delta_S2_-_L1.tex}
\end{table}
\begin{table}[htbp]
\centering
\caption{Scaling dimension for the sector $S=2^{-}, L=2$. For the ED and DMRG data, the numbers in bracket is the corresponding system size. For the $\epsilon$-expansion and large-$N$ expansion, the numbers in the bracket indicate the order of the expansion.}}
\input{Delta_Tables/Delta_S2_-_L2.tex}
\end{table}
\begin{table}[htbp]
\centering
\caption{Scaling dimension for the sector $S=2^{-}, L=3$. For the ED and DMRG data, the numbers in bracket is the corresponding system size. For the $\epsilon$-expansion and large-$N$ expansion, the numbers in the bracket indicate the order of the expansion.}}
\input{Delta_Tables/Delta_S2_-_L3.tex}
\end{table}
\begin{table}[htbp]
\centering
\caption{Scaling dimension for the sector $S=2^{-}, L=4$. For the ED and DMRG data, the numbers in bracket is the corresponding system size. For the $\epsilon$-expansion and large-$N$ expansion, the numbers in the bracket indicate the order of the expansion.}}
\input{Delta_Tables/Delta_S2_-_L4.tex}
\end{table}
\begin{table}[htbp]
\centering
\caption{Scaling dimension for the sector $S=2^{-}, L=5$. For the ED and DMRG data, the numbers in bracket is the corresponding system size. For the $\epsilon$-expansion and large-$N$ expansion, the numbers in the bracket indicate the order of the expansion.}}
\input{Delta_Tables/Delta_S2_-_L5.tex}
\end{table}
\begin{table}[htbp]
\centering
\caption{Scaling dimension for the sector $S=2^{-}, L=6$. For the ED and DMRG data, the numbers in bracket is the corresponding system size. For the $\epsilon$-expansion and large-$N$ expansion, the numbers in the bracket indicate the order of the expansion.}}
\input{Delta_Tables/Delta_S2_-_L6.tex}
\end{table}
\begin{table}[htbp]
\centering
\caption{Scaling dimension for the sector $S=2^{-}, L=7$. For the ED and DMRG data, the numbers in bracket is the corresponding system size. For the $\epsilon$-expansion and large-$N$ expansion, the numbers in the bracket indicate the order of the expansion.}}
\input{Delta_Tables/Delta_S2_-_L7.tex}
\end{table}

% ===== S = 3, parity + =====
\begin{table}[htbp]
\centering
\caption{Scaling dimension for the sector $S=3^{+}, L=0$. For the ED and DMRG data, the numbers in bracket is the corresponding system size. For the $\epsilon$-expansion and large-$N$ expansion, the numbers in the bracket indicate the order of the expansion.}}
\input{Delta_Tables/Delta_S3_+_L0.tex}
\end{table}
\begin{table}[htbp]
\centering
\caption{Scaling dimension for the sector $S=3^{+}, L=1$. For the ED and DMRG data, the numbers in bracket is the corresponding system size. For the $\epsilon$-expansion and large-$N$ expansion, the numbers in the bracket indicate the order of the expansion.}}
\input{Delta_Tables/Delta_S3_+_L1.tex}
\end{table}
\begin{table}[htbp]
\centering
\caption{Scaling dimension for the sector $S=3^{+}, L=2$. For the ED and DMRG data, the numbers in bracket is the corresponding system size. For the $\epsilon$-expansion and large-$N$ expansion, the numbers in the bracket indicate the order of the expansion.}}
\input{Delta_Tables/Delta_S3_+_L2.tex}
\end{table}
\begin{table}[htbp]
\centering
\caption{Scaling dimension for the sector $S=3^{+}, L=3$. For the ED and DMRG data, the numbers in bracket is the corresponding system size. For the $\epsilon$-expansion and large-$N$ expansion, the numbers in the bracket indicate the order of the expansion.}}
\input{Delta_Tables/Delta_S3_+_L3.tex}
\end{table}
\begin{table}[htbp]
\centering
\caption{Scaling dimension for the sector $S=3^{+}, L=4$. For the ED and DMRG data, the numbers in bracket is the corresponding system size. For the $\epsilon$-expansion and large-$N$ expansion, the numbers in the bracket indicate the order of the expansion.}}
\input{Delta_Tables/Delta_S3_+_L4.tex}
\end{table}
\begin{table}[htbp]
\centering
\caption{Scaling dimension for the sector $S=3^{+}, L=5$. For the ED and DMRG data, the numbers in bracket is the corresponding system size. For the $\epsilon$-expansion and large-$N$ expansion, the numbers in the bracket indicate the order of the expansion.}}
\input{Delta_Tables/Delta_S3_+_L5.tex}
\end{table}
\begin{table}[htbp]
\centering
\caption{Scaling dimension for the sector $S=3^{+}, L=6$. For the ED and DMRG data, the numbers in bracket is the corresponding system size. For the $\epsilon$-expansion and large-$N$ expansion, the numbers in the bracket indicate the order of the expansion.}}
\input{Delta_Tables/Delta_S3_+_L6.tex}
\end{table}
\begin{table}[htbp]
\centering
\caption{Scaling dimension for the sector $S=3^{+}, L=7$. For the ED and DMRG data, the numbers in bracket is the corresponding system size. For the $\epsilon$-expansion and large-$N$ expansion, the numbers in the bracket indicate the order of the expansion.}}
\input{Delta_Tables/Delta_S3_+_L7.tex}
\end{table}

% ===== S = 3, parity - =====
\begin{table}[htbp]
\centering
\caption{Scaling dimension for the sector $S=3^{-}, L=0$. For the ED and DMRG data, the numbers in bracket is the corresponding system size. For the $\epsilon$-expansion and large-$N$ expansion, the numbers in the bracket indicate the order of the expansion.}}
\input{Delta_Tables/Delta_S3_-_L0.tex}
\end{table}
\begin{table}[htbp]
\centering
\caption{Scaling dimension for the sector $S=3^{-}, L=1$. For the ED and DMRG data, the numbers in bracket is the corresponding system size. For the $\epsilon$-expansion and large-$N$ expansion, the numbers in the bracket indicate the order of the expansion.}}
\input{Delta_Tables/Delta_S3_-_L1.tex}
\end{table}
\begin{table}[htbp]
\centering
\caption{Scaling dimension for the sector $S=3^{-}, L=2$. For the ED and DMRG data, the numbers in bracket is the corresponding system size. For the $\epsilon$-expansion and large-$N$ expansion, the numbers in the bracket indicate the order of the expansion.}}
\input{Delta_Tables/Delta_S3_-_L2.tex}
\end{table}
\begin{table}[htbp]
\centering
\caption{Scaling dimension for the sector $S=3^{-}, L=3$. For the ED and DMRG data, the numbers in bracket is the corresponding system size. For the $\epsilon$-expansion and large-$N$ expansion, the numbers in the bracket indicate the order of the expansion.}}
\input{Delta_Tables/Delta_S3_-_L3.tex}
\end{table}
\begin{table}[htbp]
\centering
\caption{Scaling dimension for the sector $S=3^{-}, L=4$. For the ED and DMRG data, the numbers in bracket is the corresponding system size. For the $\epsilon$-expansion and large-$N$ expansion, the numbers in the bracket indicate the order of the expansion.}}
\input{Delta_Tables/Delta_S3_-_L4.tex}
\end{table}
\begin{table}[htbp]
\centering
\caption{Scaling dimension for the sector $S=3^{-}, L=5$. For the ED and DMRG data, the numbers in bracket is the corresponding system size. For the $\epsilon$-expansion and large-$N$ expansion, the numbers in the bracket indicate the order of the expansion.}}
\input{Delta_Tables/Delta_S3_-_L5.tex}
\end{table}
\begin{table}[htbp]
\centering
\caption{Scaling dimension for the sector $S=3^{-}, L=6$. For the ED and DMRG data, the numbers in bracket is the corresponding system size. For the $\epsilon$-expansion and large-$N$ expansion, the numbers in the bracket indicate the order of the expansion.}}
\input{Delta_Tables/Delta_S3_-_L6.tex}
\end{table}
\begin{table}[htbp]
\centering
\caption{Scaling dimension for the sector $S=3^{-}, L=7$. For the ED and DMRG data, the numbers in bracket is the corresponding system size. For the $\epsilon$-expansion and large-$N$ expansion, the numbers in the bracket indicate the order of the expansion.}}
\input{Delta_Tables/Delta_S3_-_L7.tex}
\end{table}

% ===== S = 4, parity + =====
\begin{table}[htbp]
\centering
\caption{Scaling dimension for the sector $S=4^{+}, L=0$. For the ED and DMRG data, the numbers in bracket is the corresponding system size. For the $\epsilon$-expansion and large-$N$ expansion, the numbers in the bracket indicate the order of the expansion.}}
\input{Delta_Tables/Delta_S4_+_L0.tex}
\end{table}
\begin{table}[htbp]
\centering
\caption{Scaling dimension for the sector $S=4^{+}, L=1$. For the ED and DMRG data, the numbers in bracket is the corresponding system size. For the $\epsilon$-expansion and large-$N$ expansion, the numbers in the bracket indicate the order of the expansion.}}
\input{Delta_Tables/Delta_S4_+_L1.tex}
\end{table}
\begin{table}[htbp]
\centering
\caption{Scaling dimension for the sector $S=4^{+}, L=2$. For the ED and DMRG data, the numbers in bracket is the corresponding system size. For the $\epsilon$-expansion and large-$N$ expansion, the numbers in the bracket indicate the order of the expansion.}}
\input{Delta_Tables/Delta_S4_+_L2.tex}
\end{table}
\begin{table}[htbp]
\centering
\caption{Scaling dimension for the sector $S=4^{+}, L=3$. For the ED and DMRG data, the numbers in bracket is the corresponding system size. For the $\epsilon$-expansion and large-$N$ expansion, the numbers in the bracket indicate the order of the expansion.}}
\input{Delta_Tables/Delta_S4_+_L3.tex}
\end{table}
\begin{table}[htbp]
\centering
\caption{Scaling dimension for the sector $S=4^{+}, L=4$. For the ED and DMRG data, the numbers in bracket is the corresponding system size. For the $\epsilon$-expansion and large-$N$ expansion, the numbers in the bracket indicate the order of the expansion.}}
\input{Delta_Tables/Delta_S4_+_L4.tex}
\end{table}
\begin{table}[htbp]
\centering
\caption{Scaling dimension for the sector $S=4^{+}, L=5$. For the ED and DMRG data, the numbers in bracket is the corresponding system size. For the $\epsilon$-expansion and large-$N$ expansion, the numbers in the bracket indicate the order of the expansion.}}
\input{Delta_Tables/Delta_S4_+_L5.tex}
\end{table}
\begin{table}[htbp]
\centering
\caption{Scaling dimension for the sector $S=4^{+}, L=6$. For the ED and DMRG data, the numbers in bracket is the corresponding system size. For the $\epsilon$-expansion and large-$N$ expansion, the numbers in the bracket indicate the order of the expansion.}}
\input{Delta_Tables/Delta_S4_+_L6.tex}
\end{table}
\begin{table}[htbp]
\centering
\caption{Scaling dimension for the sector $S=4^{+}, L=7$. For the ED and DMRG data, the numbers in bracket is the corresponding system size. For the $\epsilon$-expansion and large-$N$ expansion, the numbers in the bracket indicate the order of the expansion.}}
\input{Delta_Tables/Delta_S4_+_L7.tex}
\end{table}

% ===== S = 4, parity - =====
\begin{table}[htbp]
\centering
\caption{Scaling dimension for the sector $S=4^{-}, L=0$. For the ED and DMRG data, the numbers in bracket is the corresponding system size. For the $\epsilon$-expansion and large-$N$ expansion, the numbers in the bracket indicate the order of the expansion.}}
\input{Delta_Tables/Delta_S4_-_L0.tex}
\end{table}
\begin{table}[htbp]
\centering
\caption{Scaling dimension for the sector $S=4^{-}, L=1$. For the ED and DMRG data, the numbers in bracket is the corresponding system size. For the $\epsilon$-expansion and large-$N$ expansion, the numbers in the bracket indicate the order of the expansion.}}
\input{Delta_Tables/Delta_S4_-_L1.tex}
\end{table}
\begin{table}[htbp]
\centering
\caption{Scaling dimension for the sector $S=4^{-}, L=2$. For the ED and DMRG data, the numbers in bracket is the corresponding system size. For the $\epsilon$-expansion and large-$N$ expansion, the numbers in the bracket indicate the order of the expansion.}}
\input{Delta_Tables/Delta_S4_-_L2.tex}
\end{table}
\begin{table}[htbp]
\centering
\caption{Scaling dimension for the sector $S=4^{-}, L=3$. For the ED and DMRG data, the numbers in bracket is the corresponding system size. For the $\epsilon$-expansion and large-$N$ expansion, the numbers in the bracket indicate the order of the expansion.}}
\input{Delta_Tables/Delta_S4_-_L3.tex}
\end{table}
\begin{table}[htbp]
\centering
\caption{Scaling dimension for the sector $S=4^{-}, L=4$. For the ED and DMRG data, the numbers in bracket is the corresponding system size. For the $\epsilon$-expansion and large-$N$ expansion, the numbers in the bracket indicate the order of the expansion.}}
\input{Delta_Tables/Delta_S4_-_L4.tex}
\end{table}
\begin{table}[htbp]
\centering
\caption{Scaling dimension for the sector $S=4^{-}, L=5$. For the ED and DMRG data, the numbers in bracket is the corresponding system size. For the $\epsilon$-expansion and large-$N$ expansion, the numbers in the bracket indicate the order of the expansion.}}
\input{Delta_Tables/Delta_S4_-_L5.tex}
\end{table}
\begin{table}[htbp]
\centering
\caption{Scaling dimension for the sector $S=4^{-}, L=6$. For the ED and DMRG data, the numbers in bracket is the corresponding system size. For the $\epsilon$-expansion and large-$N$ expansion, the numbers in the bracket indicate the order of the expansion.}}
\input{Delta_Tables/Delta_S4_-_L6.tex}
\end{table}
\begin{table}[htbp]
\centering
\caption{Scaling dimension for the sector $S=4^{-}, L=7$. For the ED and DMRG data, the numbers in bracket is the corresponding system size. For the $\epsilon$-expansion and large-$N$ expansion, the numbers in the bracket indicate the order of the expansion.}}
\input{Delta_Tables/Delta_S4_-_L7.tex}
\end{table}

% ===== S = 5, parity + =====
\begin{table}[htbp]
\centering
\caption{Scaling dimension for the sector $S=5^{+}, L=0$. For the ED and DMRG data, the numbers in bracket is the corresponding system size. For the $\epsilon$-expansion and large-$N$ expansion, the numbers in the bracket indicate the order of the expansion.}}
\input{Delta_Tables/Delta_S5_+_L0.tex}
\end{table}
\begin{table}[htbp]
\centering
\caption{Scaling dimension for the sector $S=5^{+}, L=1$. For the ED and DMRG data, the numbers in bracket is the corresponding system size. For the $\epsilon$-expansion and large-$N$ expansion, the numbers in the bracket indicate the order of the expansion.}}
\input{Delta_Tables/Delta_S5_+_L1.tex}
\end{table}
\begin{table}[htbp]
\centering
\caption{Scaling dimension for the sector $S=5^{+}, L=2$. For the ED and DMRG data, the numbers in bracket is the corresponding system size. For the $\epsilon$-expansion and large-$N$ expansion, the numbers in the bracket indicate the order of the expansion.}}
\input{Delta_Tables/Delta_S5_+_L2.tex}
\end{table}
\begin{table}[htbp]
\centering
\caption{Scaling dimension for the sector $S=5^{+}, L=3$. For the ED and DMRG data, the numbers in bracket is the corresponding system size. For the $\epsilon$-expansion and large-$N$ expansion, the numbers in the bracket indicate the order of the expansion.}}
\input{Delta_Tables/Delta_S5_+_L3.tex}
\end{table}
\begin{table}[htbp]
\centering
\caption{Scaling dimension for the sector $S=5^{+}, L=4$. For the ED and DMRG data, the numbers in bracket is the corresponding system size. For the $\epsilon$-expansion and large-$N$ expansion, the numbers in the bracket indicate the order of the expansion.}}
\input{Delta_Tables/Delta_S5_+_L4.tex}
\end{table}
\begin{table}[htbp]
\centering
\caption{Scaling dimension for the sector $S=5^{+}, L=5$. For the ED and DMRG data, the numbers in bracket is the corresponding system size. For the $\epsilon$-expansion and large-$N$ expansion, the numbers in the bracket indicate the order of the expansion.}}
\input{Delta_Tables/Delta_S5_+_L5.tex}
\end{table}
\begin{table}[htbp]
\centering
\caption{Scaling dimension for the sector $S=5^{+}, L=6$. For the ED and DMRG data, the numbers in bracket is the corresponding system size. For the $\epsilon$-expansion and large-$N$ expansion, the numbers in the bracket indicate the order of the expansion.}}
\input{Delta_Tables/Delta_S5_+_L6.tex}
\end{table}
\begin{table}[htbp]
\centering
\caption{Scaling dimension for the sector $S=5^{+}, L=7$. For the ED and DMRG data, the numbers in bracket is the corresponding system size. For the $\epsilon$-expansion and large-$N$ expansion, the numbers in the bracket indicate the order of the expansion.}}
\input{Delta_Tables/Delta_S5_+_L7.tex}
\end{table}

% ===== S = 5, parity - =====
\begin{table}[htbp]
\centering
\caption{Scaling dimension for the sector $S=5^{-}, L=0$. For the ED and DMRG data, the numbers in bracket is the corresponding system size. For the $\epsilon$-expansion and large-$N$ expansion, the numbers in the bracket indicate the order of the expansion.}}
\input{Delta_Tables/Delta_S5_-_L0.tex}
\end{table}
\begin{table}[htbp]
\centering
\caption{Scaling dimension for the sector $S=5^{-}, L=1$. For the ED and DMRG data, the numbers in bracket is the corresponding system size. For the $\epsilon$-expansion and large-$N$ expansion, the numbers in the bracket indicate the order of the expansion.}}
\input{Delta_Tables/Delta_S5_-_L1.tex}
\end{table}
\begin{table}[htbp]
\centering
\caption{Scaling dimension for the sector $S=5^{-}, L=2$. For the ED and DMRG data, the numbers in bracket is the corresponding system size. For the $\epsilon$-expansion and large-$N$ expansion, the numbers in the bracket indicate the order of the expansion.}}
\input{Delta_Tables/Delta_S5_-_L2.tex}
\end{table}
\begin{table}[htbp]
\centering
\caption{Scaling dimension for the sector $S=5^{-}, L=3$. For the ED and DMRG data, the numbers in bracket is the corresponding system size. For the $\epsilon$-expansion and large-$N$ expansion, the numbers in the bracket indicate the order of the expansion.}}
\input{Delta_Tables/Delta_S5_-_L3.tex}
\end{table}
\begin{table}[htbp]
\centering
\caption{Scaling dimension for the sector $S=5^{-}, L=4$. For the ED and DMRG data, the numbers in bracket is the corresponding system size. For the $\epsilon$-expansion and large-$N$ expansion, the numbers in the bracket indicate the order of the expansion.}}
\input{Delta_Tables/Delta_S5_-_L4.tex}
\end{table}
\begin{table}[htbp]
\centering
\caption{Scaling dimension for the sector $S=5^{-}, L=5$. For the ED and DMRG data, the numbers in bracket is the corresponding system size. For the $\epsilon$-expansion and large-$N$ expansion, the numbers in the bracket indicate the order of the expansion.}}
\input{Delta_Tables/Delta_S5_-_L5.tex}
\end{table}
\begin{table}[htbp]
\centering
\caption{Scaling dimension for the sector $S=5^{-}, L=6$. For the ED and DMRG data, the numbers in bracket is the corresponding system size. For the $\epsilon$-expansion and large-$N$ expansion, the numbers in the bracket indicate the order of the expansion.}}
\input{Delta_Tables/Delta_S5_-_L6.tex}
\end{table}
\begin{table}[htbp]
\centering
\caption{Scaling dimension for the sector $S=5^{-}, L=7$. For the ED and DMRG data, the numbers in bracket is the corresponding system size. For the $\epsilon$-expansion and large-$N$ expansion, the numbers in the bracket indicate the order of the expansion.}}
\input{Delta_Tables/Delta_S5_-_L7.tex}
\end{table}

% ===== S = 6, parity + =====
\begin{table}[htbp]
\centering
\caption{Scaling dimension for the sector $S=6^{+}, L=0$. For the ED and DMRG data, the numbers in bracket is the corresponding system size. For the $\epsilon$-expansion and large-$N$ expansion, the numbers in the bracket indicate the order of the expansion.}}
\input{Delta_Tables/Delta_S6_+_L0.tex}
\end{table}
\begin{table}[htbp]
\centering
\caption{Scaling dimension for the sector $S=6^{+}, L=1$. For the ED and DMRG data, the numbers in bracket is the corresponding system size. For the $\epsilon$-expansion and large-$N$ expansion, the numbers in the bracket indicate the order of the expansion.}}
\input{Delta_Tables/Delta_S6_+_L1.tex}
\end{table}
\begin{table}[htbp]
\centering
\caption{Scaling dimension for the sector $S=6^{+}, L=2$. For the ED and DMRG data, the numbers in bracket is the corresponding system size. For the $\epsilon$-expansion and large-$N$ expansion, the numbers in the bracket indicate the order of the expansion.}}
\input{Delta_Tables/Delta_S6_+_L2.tex}
\end{table}
\begin{table}[htbp]
\centering
\caption{Scaling dimension for the sector $S=6^{+}, L=3$. For the ED and DMRG data, the numbers in bracket is the corresponding system size. For the $\epsilon$-expansion and large-$N$ expansion, the numbers in the bracket indicate the order of the expansion.}}
\input{Delta_Tables/Delta_S6_+_L3.tex}
\end{table}
\begin{table}[htbp]
\centering
\caption{Scaling dimension for the sector $S=6^{+}, L=4$. For the ED and DMRG data, the numbers in bracket is the corresponding system size. For the $\epsilon$-expansion and large-$N$ expansion, the numbers in the bracket indicate the order of the expansion.}}
\input{Delta_Tables/Delta_S6_+_L4.tex}
\end{table}
\begin{table}[htbp]
\centering
\caption{Scaling dimension for the sector $S=6^{+}, L=5$. For the ED and DMRG data, the numbers in bracket is the corresponding system size. For the $\epsilon$-expansion and large-$N$ expansion, the numbers in the bracket indicate the order of the expansion.}}
\input{Delta_Tables/Delta_S6_+_L5.tex}
\end{table}
\begin{table}[htbp]
\centering
\caption{Scaling dimension for the sector $S=6^{+}, L=6$. For the ED and DMRG data, the numbers in bracket is the corresponding system size. For the $\epsilon$-expansion and large-$N$ expansion, the numbers in the bracket indicate the order of the expansion.}}
\input{Delta_Tables/Delta_S6_+_L6.tex}
\end{table}
\begin{table}[htbp]
\centering
\caption{Scaling dimension for the sector $S=6^{+}, L=7$. For the ED and DMRG data, the numbers in bracket is the corresponding system size. For the $\epsilon$-expansion and large-$N$ expansion, the numbers in the bracket indicate the order of the expansion.}}
\input{Delta_Tables/Delta_S6_+_L7.tex}
\end{table}

% ===== S = 6, parity - =====
\begin{table}[htbp]
\centering
\caption{Scaling dimension for the sector $S=6^{-}, L=0$. For the ED and DMRG data, the numbers in bracket is the corresponding system size. For the $\epsilon$-expansion and large-$N$ expansion, the numbers in the bracket indicate the order of the expansion.}}
\input{Delta_Tables/Delta_S6_-_L0.tex}
\end{table}
\begin{table}[htbp]
\centering
\caption{Scaling dimension for the sector $S=6^{-}, L=1$. For the ED and DMRG data, the numbers in bracket is the corresponding system size. For the $\epsilon$-expansion and large-$N$ expansion, the numbers in the bracket indicate the order of the expansion.}}
\input{Delta_Tables/Delta_S6_-_L1.tex}
\end{table}
\begin{table}[htbp]
\centering
\caption{Scaling dimension for the sector $S=6^{-}, L=2$. For the ED and DMRG data, the numbers in bracket is the corresponding system size. For the $\epsilon$-expansion and large-$N$ expansion, the numbers in the bracket indicate the order of the expansion.}}
\input{Delta_Tables/Delta_S6_-_L2.tex}
\end{table}
\begin{table}[htbp]
\centering
\caption{Scaling dimension for the sector $S=6^{-}, L=3$. For the ED and DMRG data, the numbers in bracket is the corresponding system size. For the $\epsilon$-expansion and large-$N$ expansion, the numbers in the bracket indicate the order of the expansion.}}
\input{Delta_Tables/Delta_S6_-_L3.tex}
\end{table}
\begin{table}[htbp]
\centering
\caption{Scaling dimension for the sector $S=6^{-}, L=4$. For the ED and DMRG data, the numbers in bracket is the corresponding system size. For the $\epsilon$-expansion and large-$N$ expansion, the numbers in the bracket indicate the order of the expansion.}}
\input{Delta_Tables/Delta_S6_-_L4.tex}
\end{table}
\begin{table}[htbp]
\centering
\caption{Scaling dimension for the sector $S=6^{-}, L=5$. For the ED and DMRG data, the numbers in bracket is the corresponding system size. For the $\epsilon$-expansion and large-$N$ expansion, the numbers in the bracket indicate the order of the expansion.}}
\input{Delta_Tables/Delta_S6_-_L5.tex}
\end{table}
\begin{table}[htbp]
\centering
\caption{Scaling dimension for the sector $S=6^{-}, L=6$. For the ED and DMRG data, the numbers in bracket is the corresponding system size. For the $\epsilon$-expansion and large-$N$ expansion, the numbers in the bracket indicate the order of the expansion.}}
\input{Delta_Tables/Delta_S6_-_L6.tex}
\end{table}
\begin{table}[htbp]
\centering
\caption{Scaling dimension for the sector $S=6^{-}, L=7$. For the ED and DMRG data, the numbers in bracket is the corresponding system size. For the $\epsilon$-expansion and large-$N$ expansion, the numbers in the bracket indicate the order of the expansion.}}
\input{Delta_Tables/Delta_S6_-_L7.tex}
\end{table}

% ===== S = 7, parity + =====
\begin{table}[htbp]
\centering
\caption{Scaling dimension for the sector $S=7^{+}, L=0$. For the ED and DMRG data, the numbers in bracket is the corresponding system size. For the $\epsilon$-expansion and large-$N$ expansion, the numbers in the bracket indicate the order of the expansion.}}
\input{Delta_Tables/Delta_S7_+_L0.tex}
\end{table}
\begin{table}[htbp]
\centering
\caption{Scaling dimension for the sector $S=7^{+}, L=1$. For the ED and DMRG data, the numbers in bracket is the corresponding system size. For the $\epsilon$-expansion and large-$N$ expansion, the numbers in the bracket indicate the order of the expansion.}}
\input{Delta_Tables/Delta_S7_+_L1.tex}
\end{table}
\begin{table}[htbp]
\centering
\caption{Scaling dimension for the sector $S=7^{+}, L=2$. For the ED and DMRG data, the numbers in bracket is the corresponding system size. For the $\epsilon$-expansion and large-$N$ expansion, the numbers in the bracket indicate the order of the expansion.}}
\input{Delta_Tables/Delta_S7_+_L2.tex}
\end{table}
\begin{table}[htbp]
\centering
\caption{Scaling dimension for the sector $S=7^{+}, L=3$. For the ED and DMRG data, the numbers in bracket is the corresponding system size. For the $\epsilon$-expansion and large-$N$ expansion, the numbers in the bracket indicate the order of the expansion.}}
\input{Delta_Tables/Delta_S7_+_L3.tex}
\end{table}
\begin{table}[htbp]
\centering
\caption{Scaling dimension for the sector $S=7^{+}, L=4$. For the ED and DMRG data, the numbers in bracket is the corresponding system size. For the $\epsilon$-expansion and large-$N$ expansion, the numbers in the bracket indicate the order of the expansion.}}
\input{Delta_Tables/Delta_S7_+_L4.tex}
\end{table}
\begin{table}[htbp]
\centering
\caption{Scaling dimension for the sector $S=7^{+}, L=5$. For the ED and DMRG data, the numbers in bracket is the corresponding system size. For the $\epsilon$-expansion and large-$N$ expansion, the numbers in the bracket indicate the order of the expansion.}}
\input{Delta_Tables/Delta_S7_+_L5.tex}
\end{table}
\begin{table}[htbp]
\centering
\caption{Scaling dimension for the sector $S=7^{+}, L=6$. For the ED and DMRG data, the numbers in bracket is the corresponding system size. For the $\epsilon$-expansion and large-$N$ expansion, the numbers in the bracket indicate the order of the expansion.}}
\input{Delta_Tables/Delta_S7_+_L6.tex}
\end{table}
\begin{table}[htbp]
\centering
\caption{Scaling dimension for the sector $S=7^{+}, L=7$. For the ED and DMRG data, the numbers in bracket is the corresponding system size. For the $\epsilon$-expansion and large-$N$ expansion, the numbers in the bracket indicate the order of the expansion.}}
\input{Delta_Tables/Delta_S7_+_L7.tex}
\end{table}

% ===== S = 7, parity - =====
\begin{table}[htbp]
\centering
\caption{Scaling dimension for the sector $S=7^{-}, L=0$. For the ED and DMRG data, the numbers in bracket is the corresponding system size. For the $\epsilon$-expansion and large-$N$ expansion, the numbers in the bracket indicate the order of the expansion.}}
\input{Delta_Tables/Delta_S7_-_L0.tex}
\end{table}
\begin{table}[htbp]
\centering
\caption{Scaling dimension for the sector $S=7^{-}, L=1$. For the ED and DMRG data, the numbers in bracket is the corresponding system size. For the $\epsilon$-expansion and large-$N$ expansion, the numbers in the bracket indicate the order of the expansion.}}
\input{Delta_Tables/Delta_S7_-_L1.tex}
\end{table}
\begin{table}[htbp]
\centering
\caption{Scaling dimension for the sector $S=7^{-}, L=2$. For the ED and DMRG data, the numbers in bracket is the corresponding system size. For the $\epsilon$-expansion and large-$N$ expansion, the numbers in the bracket indicate the order of the expansion.}}
\input{Delta_Tables/Delta_S7_-_L2.tex}
\end{table}
\begin{table}[htbp]
\centering
\caption{Scaling dimension for the sector $S=7^{-}, L=3$. For the ED and DMRG data, the numbers in bracket is the corresponding system size. For the $\epsilon$-expansion and large-$N$ expansion, the numbers in the bracket indicate the order of the expansion.}}
\input{Delta_Tables/Delta_S7_-_L3.tex}
\end{table}
\begin{table}[htbp]
\centering
\caption{Scaling dimension for the sector $S=7^{-}, L=4$. For the ED and DMRG data, the numbers in bracket is the corresponding system size. For the $\epsilon$-expansion and large-$N$ expansion, the numbers in the bracket indicate the order of the expansion.}}
\input{Delta_Tables/Delta_S7_-_L4.tex}
\end{table}
\begin{table}[htbp]
\centering
\caption{Scaling dimension for the sector $S=7^{-}, L=5$. For the ED and DMRG data, the numbers in bracket is the corresponding system size. For the $\epsilon$-expansion and large-$N$ expansion, the numbers in the bracket indicate the order of the expansion.}}
\input{Delta_Tables/Delta_S7_-_L5.tex}
\end{table}
\begin{table}[htbp]
\centering
\caption{Scaling dimension for the sector $S=7^{-}, L=6$. For the ED and DMRG data, the numbers in bracket is the corresponding system size. For the $\epsilon$-expansion and large-$N$ expansion, the numbers in the bracket indicate the order of the expansion.}}
\input{Delta_Tables/Delta_S7_-_L6.tex}
\end{table}
\begin{table}[htbp]
\centering
\caption{Scaling dimension for the sector $S=7^{-}, L=7$. For the ED and DMRG data, the numbers in bracket is the corresponding system size. For the $\epsilon$-expansion and large-$N$ expansion, the numbers in the bracket indicate the order of the expansion.}}
\input{Delta_Tables/Delta_S7_-_L7.tex}
\end{table}


==> OPE_Tables/OPE_Table_S0_+.tex <==
\begin{tabular}{|c|c|c|c||c|c|c|c|}
\hline
$L$ & Index & $\lambda_{\mathcal{O}\varepsilon\mathcal{O}}$ (ED) & $\lambda_{\mathcal{O}\varepsilon\mathcal{O}}$ (DMRG) & $L$ & Index & $\lambda_{\mathcal{O}\varepsilon\mathcal{O}}$ (ED) & $\lambda_{\mathcal{O}\varepsilon\mathcal{O}}$ (DMRG) \\
\hline
0 & 0 ($\Omega$) & 0.0000 $(N=10)$ & 0.0000 $(N=18)$ & 2 & 3 & 1.1578 $(N=10)$ & -- \\ \hline
0 & 1 ($\varepsilon$) & 0.5328 $(N=10)$ & 0.4803 $(N=18)$ & 2 & 4 & 1.1114 $(N=10)$ & -- \\ \hline
0 & 2 ($\partial\partial\varepsilon^{(0)}$) & 0.6198 $(N=10)$ & -- & 3 & 0 ($\partial T_{\mu \nu}$) & 0.3946 $(N=10)$ & 0.3814 $(N=18)$ \\ \hline
0 & 3 ($\varepsilon'$) & 1.0795 $(N=10)$ & -- & 3 & 1 ($\partial\partial\partial\varepsilon^{(3)}$) & 0.2062 $(N=10)$ & -- \\ \hline
0 & 4 & 1.1806 $(N=10)$ & -- & 3 & 2 & 0.8304 $(N=10)$ & -- \\ \hline
1 & 0 ($\partial\varepsilon$) & 0.4027 $(N=10)$ & 0.3662 $(N=18)$ & 4 & 0 & 0.3609 $(N=10)$ & -- \\ \hline
1 & 1 ($\partial\partial\partial\varepsilon^{(1)}$) & 0.9653 $(N=10)$ & -- & 4 & 1 & 0.2667 $(N=10)$ & -- \\ \hline
1 & 2 & 0.6542 $(N=10)$ & -- & 4 & 2 & 0.4987 $(N=10)$ & -- \\ \hline
2 & 0 ($T_{\mu \nu}$) & 0.4724 $(N=10)$ & 0.4611 $(N=18)$ & 5 & 0 & 0.3472 $(N=10)$ & -- \\ \hline
2 & 1 ($\partial\partial\varepsilon^{(2)}$) & 0.2964 $(N=10)$ & 0.2931 $(N=18)$ & 6 & 0 & 0.3446 $(N=9)$ & -- \\ \hline
2 & 2 ($\epsilon \partial T_{\mu \nu}$) & 0.3783 $(N=10)$ & -- & 7 & 0 & 0.3623 $(N=9)$ & -- \\ \hline
\end{tabular}

==> OPE_Tables/OPE_Table_S0_-.tex <==
\begin{tabular}{|c|c|c|c||c|c|c|c|}
\hline
$L$ & Index & $\lambda_{\mathcal{O}\varepsilon\mathcal{O}}$ (ED) & $\lambda_{\mathcal{O}\varepsilon\mathcal{O}}$ (DMRG) & $L$ & Index & $\lambda_{\mathcal{O}\varepsilon\mathcal{O}}$ (ED) & $\lambda_{\mathcal{O}\varepsilon\mathcal{O}}$ (DMRG) \\
\hline
0 & 0 ($\partial \varepsilon_{\mu}^{(0)}$) & 0.7463 $(N=10)$ & -- & 4 & 0 & 0.7643 $(N=10)$ & -- \\ \hline
1 & 0 ($\varepsilon_{\mu}$) & 1.1328 $(N=10)$ & 1.0491 $(N=18)$ & 4 & 1 & 0.7298 $(N=10)$ & -- \\ \hline
1 & 1 ($\epsilon \partial \varepsilon_{\mu}$) & 0.9388 $(N=10)$ & -- & 5 & 0 & 0.7064 $(N=10)$ & -- \\ \hline
1 & 2 & 0.6619 $(N=10)$ & -- & 5 & 1 & 0.6417 $(N=10)$ & -- \\ \hline
2 & 0 ($\partial \varepsilon_{\mu}^{(2)}$) & 1.0053 $(N=10)$ & -- & 6 & 0 & 0.6700 $(N=10)$ & -- \\ \hline
2 & 1 & 0.6335 $(N=10)$ & -- & 7 & 0 & 0.6735 $(N=9)$ & -- \\ \hline
2 & 2 & 0.7066 $(N=10)$ & -- & 7 & 1 & 0.6165 $(N=9)$ & -- \\ \hline
3 & 0 & 0.8487 $(N=10)$ & -- & 8 & 0 & 0.6109 $(N=9)$ & -- \\ \hline
3 & 1 & 0.8576 $(N=10)$ & -- & 9 & 0 & 0.6078 $(N=9)$ & -- \\ \hline
3 & 2 & 0.7258 $(N=10)$ & -- &  & & &  \\ \hline
\end{tabular}

==> OPE_Tables/OPE_Table_S1_+.tex <==
\begin{tabular}{|c|c|c|c||c|c|c|c|}
\hline
$L$ & Index & $\lambda_{\mathcal{O}\varepsilon\mathcal{O}}$ (ED) & $\lambda_{\mathcal{O}\varepsilon\mathcal{O}}$ (DMRG) & $L$ & Index & $\lambda_{\mathcal{O}\varepsilon\mathcal{O}}$ (ED) & $\lambda_{\mathcal{O}\varepsilon\mathcal{O}}$ (DMRG) \\
\hline
0 & 0 & 1.2750 $(N=5)$ & -- & 2 & 5 & 1.3313 $(N=10)$ & -- \\ \hline
0 & 1 & 1.2261 $(N=5)$ & -- & 2 & 6 & 0.4374 $(N=10)$ & -- \\ \hline
0 & 2 & 1.0778 $(N=5)$ & -- & 3 & 0 ($\partial \partial j_{\mu}$) & 0.4589 $(N=10)$ & 0.4873 $(N=18)$ \\ \hline
1 & 0 ($j_{\mu}$) & 0.7509 $(N=10)$ & 0.7387 $(N=18)$ & 3 & 1 & 0.2606 $(N=10)$ & 0.2388 $(N=18)$ \\ \hline
1 & 1 ($\epsilon \partial j_{\mu}$) & 0.4434 $(N=10)$ & 0.3815 $(N=18)$ & 3 & 2 & 0.3685 $(N=10)$ & -- \\ \hline
1 & 2 ($\phi_{\mu}$) & 0.3503 $(N=10)$ & 0.2547 $(N=18)$ & 3 & 3 & 1.2517 $(N=10)$ & -- \\ \hline
1 & 3 & 1.3036 $(N=10)$ & -- & 3 & 4 & 1.0977 $(N=10)$ & -- \\ \hline
1 & 4 & 1.4510 $(N=10)$ & -- & 3 & 5 & 1.2016 $(N=10)$ & -- \\ \hline
1 & 5 & 1.3745 $(N=10)$ & -- & 4 & 0 ($\partial \partial \partial j_{\mu}$) & 0.3532 $(N=10)$ & 0.3742 $(N=18)$ \\ \hline
1 & 6 & 0.9008 $(N=10)$ & -- & 4 & 1 & 0.4091 $(N=10)$ & -- \\ \hline
2 & 0 ($\partial j_{\mu}$) & 0.6004 $(N=10)$ & 0.6187 $(N=18)$ & 5 & 0 & 0.2907 $(N=10)$ & -- \\ \hline
2 & 1 ($\epsilon \partial j_{\mu}$) & 0.3535 $(N=10)$ & 0.3064 $(N=18)$ & 6 & 0 & 0.2662 $(N=10)$ & -- \\ \hline
2 & 2 & 1.4029 $(N=10)$ & -- & 7 & 0 & 0.2628 $(N=10)$ & -- \\ \hline
2 & 3 & 1.1721 $(N=10)$ & -- & 8 & 0 & 0.2669 $(N=10)$ & -- \\ \hline
2 & 4 & 1.0266 $(N=10)$ & -- & 9 & 0 & 0.2716 $(N=10)$ & -- \\ \hline
\end{tabular}

==> OPE_Tables/OPE_Table_S1_-.tex <==
\begin{tabular}{|c|c|c|c||c|c|c|c|}
\hline
$L$ & Index & $\lambda_{\mathcal{O}\varepsilon\mathcal{O}}$ (ED) & $\lambda_{\mathcal{O}\varepsilon\mathcal{O}}$ (DMRG) & $L$ & Index & $\lambda_{\mathcal{O}\varepsilon\mathcal{O}}$ (ED) & $\lambda_{\mathcal{O}\varepsilon\mathcal{O}}$ (DMRG) \\
\hline
0 & 0 ($\sigma$) & 0.5250 $(N=10)$ & 0.5250 $(N=18)$ & 2 & 6 & 0.6672 $(N=10)$ & -- \\ \hline
0 & 1 ($\partial \partial \sigma^{(0)}$) & 1.0228 $(N=10)$ & -- & 2 & 7 & 0.6695 $(N=10)$ & -- \\ \hline
0 & 2 ($\sigma'$) & 0.8717 $(N=10)$ & -- & 3 & 0 ($\partial \partial \partial \sigma^{(3)}$) & 0.1111 $(N=10)$ & 0.0791 $(N=18)$ \\ \hline
0 & 3 ($\partial \partial \partial \partial \sigma^{(0)}$) & 0.8632 $(N=10)$ & -- & 3 & 1 & 0.6271 $(N=10)$ & -- \\ \hline
1 & 0 ($\partial \sigma$) & 0.1474 $(N=10)$ & 0.1474 $(N=18)$ & 3 & 2 & 0.6891 $(N=10)$ & -- \\ \hline
1 & 1 ($\sigma_{\mu}$) & 0.9628 $(N=10)$ & 0.9021 $(N=18)$ & 3 & 3 & 0.7616 $(N=10)$ & -- \\ \hline
1 & 2 ($\partial \partial \partial \sigma^{(1)}$) & 0.8720 $(N=10)$ & 0.8196 $(N=18)$ & 3 & 4 & 0.5298 $(N=10)$ & -- \\ \hline
1 & 3 & 0.7954 $(N=10)$ & 0.7238 $(N=18)$ & 3 & 5 & 0.6363 $(N=10)$ & -- \\ \hline
1 & 4 & 0.7206 $(N=10)$ & -- & 4 & 0 & 0.1820 $(N=10)$ & -- \\ \hline
1 & 5 & 0.7099 $(N=10)$ & -- & 4 & 1 & 0.3437 $(N=10)$ & -- \\ \hline
1 & 6 & 0.6677 $(N=10)$ & -- & 4 & 2 & 0.5510 $(N=10)$ & -- \\ \hline
2 & 0 ($\partial \partial \sigma^{(2)}$) & 0.0542 $(N=10)$ & 0.0669 $(N=18)$ & 5 & 0 & 0.1599 $(N=10)$ & -- \\ \hline
2 & 1 & 0.9316 $(N=10)$ & 0.9482 $(N=18)$ & 5 & 1 & 0.5442 $(N=10)$ & -- \\ \hline
2 & 2 & 0.8268 $(N=10)$ & 0.8000 $(N=18)$ & 6 & 0 & 0.1289 $(N=10)$ & -- \\ \hline
2 & 3 & 0.8181 $(N=10)$ & -- & 7 & 0 & 0.1198 $(N=10)$ & -- \\ \hline
2 & 4 & 0.7301 $(N=10)$ & -- & 8 & 0 & 0.1252 $(N=10)$ & -- \\ \hline
2 & 5 & 0.6995 $(N=10)$ & -- & 9 & 0 & 0.1344 $(N=10)$ & -- \\ \hline
\end{tabular}

==> OPE_Tables/OPE_Table_S2_+.tex <==
\begin{tabular}{|c|c|c|c||c|c|c|c|}
\hline
$L$ & Index & $\lambda_{\mathcal{O}\varepsilon\mathcal{O}}$ (ED) & $\lambda_{\mathcal{O}\varepsilon\mathcal{O}}$ (DMRG) & $L$ & Index & $\lambda_{\mathcal{O}\varepsilon\mathcal{O}}$ (ED) & $\lambda_{\mathcal{O}\varepsilon\mathcal{O}}$ (DMRG) \\
\hline
0 & 0 ($t_{(2)}$) & 0.9840 $(N=10)$ & 0.9871 $(N=18)$ & 2 & 5 & 1.2779 $(N=10)$ & -- \\ \hline
0 & 1 ($\partial\partial t_{(2)}^{(0)}$) & 0.8460 $(N=10)$ & 0.4774 $(N=18)$ & 2 & 6 & 1.2345 $(N=10)$ & -- \\ \hline
0 & 2 ($t_{(2)}'$) & 0.8848 $(N=10)$ & 1.2059 $(N=18)$ & 3 & 0 & 0.3296 $(N=10)$ & 0.3188 $(N=18)$ \\ \hline
0 & 3 ($t_{(2)}''$) & 1.4009 $(N=10)$ & -- & 3 & 1 & 0.4057 $(N=10)$ & -- \\ \hline
1 & 0 ($\partial t_{(2)}$) & 0.6646 $(N=10)$ & 0.6780 $(N=18)$ & 3 & 2 & 1.2131 $(N=10)$ & -- \\ \hline
1 & 1 ($\partial\partial\partial t_{(2)}^{(1)}$) & 1.3995 $(N=10)$ & -- & 3 & 3 & 1.1945 $(N=10)$ & -- \\ \hline
1 & 2 & 1.1314 $(N=10)$ & -- & 3 & 4 & 0.9792 $(N=10)$ & -- \\ \hline
1 & 3 & 0.5319 $(N=10)$ & -- & 4 & 0 & 0.5132 $(N=10)$ & -- \\ \hline
1 & 4 & 1.0561 $(N=10)$ & -- & 4 & 1 & 0.2633 $(N=10)$ & -- \\ \hline
2 & 0 ($t'_{(2)\mu\nu}$) & 0.3745 $(N=10)$ & 0.3817 $(N=18)$ & 5 & 0 & 0.5483 $(N=10)$ & -- \\ \hline
2 & 1 ($\partial\partial t_{(2)}^{(2)}$) & 0.4912 $(N=10)$ & 0.5409 $(N=18)$ & 6 & 0 & 0.5071 $(N=9)$ & -- \\ \hline
2 & 2 & 0.9195 $(N=10)$ & -- & 7 & 0 & 0.5204 $(N=9)$ & -- \\ \hline
2 & 3 & 0.8937 $(N=10)$ & -- & 8 & 0 & 0.5403 $(N=9)$ & -- \\ \hline
2 & 4 & 1.2309 $(N=10)$ & -- &  & & &  \\ \hline
\end{tabular}

==> OPE_Tables/OPE_Table_S2_-.tex <==
\begin{tabular}{|c|c|c|c||c|c|c|c|}
\hline
$L$ & Index & $\lambda_{\mathcal{O}\varepsilon\mathcal{O}}$ (ED) & $\lambda_{\mathcal{O}\varepsilon\mathcal{O}}$ (DMRG) & $L$ & Index & $\lambda_{\mathcal{O}\varepsilon\mathcal{O}}$ (ED) & $\lambda_{\mathcal{O}\varepsilon\mathcal{O}}$ (DMRG) \\
\hline
0 & 0 ($\partial t_{(2)\mu}^{(0)}$) & 0.9077 $(N=10)$ & -- & 3 & 1 & 0.8682 $(N=10)$ & -- \\ \hline
1 & 0 ($t_{(2)\mu}$) & 1.2306 $(N=10)$ & 1.2227 $(N=18)$ & 3 & 2 & 0.7153 $(N=10)$ & -- \\ \hline
1 & 1 ($\epsilon \partial t_{(2)\mu}^{(1)}$) & 0.9478 $(N=10)$ & 0.9248 $(N=18)$ & 3 & 3 & 0.7119 $(N=10)$ & -- \\ \hline
1 & 2 & 0.7424 $(N=10)$ & -- & 4 & 0 & 0.8546 $(N=10)$ & -- \\ \hline
1 & 3 & 0.7788 $(N=10)$ & -- & 4 & 1 & 0.7455 $(N=10)$ & -- \\ \hline
1 & 4 & 0.7091 $(N=10)$ & -- & 5 & 0 & 0.7895 $(N=10)$ & -- \\ \hline
2 & 0 ($t'_{(2)\mu\nu}$) & 1.0474 $(N=10)$ & 1.0120 $(N=18)$ & 5 & 1 & 0.6659 $(N=10)$ & -- \\ \hline
2 & 1 ($\partial t_{(2)\mu}^{(2)}$) & 1.0289 $(N=10)$ & 1.0384 $(N=18)$ & 6 & 0 & 0.7567 $(N=10)$ & -- \\ \hline
2 & 2 & 0.8295 $(N=10)$ & -- & 7 & 0 & 0.7455 $(N=10)$ & -- \\ \hline
2 & 3 & 0.7440 $(N=10)$ & -- & 8 & 0 & 0.7436 $(N=10)$ & -- \\ \hline
2 & 4 & 0.7721 $(N=10)$ & -- & 9 & 0 & 0.7441 $(N=10)$ & -- \\ \hline
3 & 0 & 0.9482 $(N=10)$ & -- & 10 & 0 & 0.5039 $(N=10)$ & -- \\ \hline
\end{tabular}

==> OPE_Tables/OPE_Table_S3_+.tex <==
\begin{tabular}{|c|c|c|c||c|c|c|c|}
\hline
$L$ & Index & $\lambda_{\mathcal{O}\varepsilon\mathcal{O}}$ (ED) & $\lambda_{\mathcal{O}\varepsilon\mathcal{O}}$ (DMRG) & $L$ & Index & $\lambda_{\mathcal{O}\varepsilon\mathcal{O}}$ (ED) & $\lambda_{\mathcal{O}\varepsilon\mathcal{O}}$ (DMRG) \\
\hline
0 & 0 ($\partial \chi_{(3)\mu}^{(0)}$) & 1.3526 $(N=10)$ & -- & 3 & 1 & 1.3394 $(N=10)$ & -- \\ \hline
1 & 0 ($\chi_{(3)\mu}$) & 1.6604 $(N=10)$ & 1.6521 $(N=18)$ & 4 & 0 & 1.3772 $(N=7)$ & -- \\ \hline
1 & 1 ($\epsilon \partial \chi_{(3)\mu}^{(1)}$) & 1.3858 $(N=10)$ & -- & 5 & 0 & 1.3746 $(N=6)$ & -- \\ \hline
2 & 0 ($\chi_{(3)\mu\nu}$) & 1.5140 $(N=10)$ & -- & 9 & 0 & 0.9694 $(N=9)$ & -- \\ \hline
2 & 1 ($\partial \chi_{(3)\mu}^{(2)}$) & 1.4536 $(N=10)$ & -- & 10 & 0 & 0.9525 $(N=10)$ & -- \\ \hline
3 & 0 & 1.3815 $(N=10)$ & -- &  & & &  \\ \hline
\end{tabular}

==> OPE_Tables/OPE_Table_S3_-.tex <==
\begin{tabular}{|c|c|c|c||c|c|c|c|}
\hline
$L$ & Index & $\lambda_{\mathcal{O}\varepsilon\mathcal{O}}$ (ED) & $\lambda_{\mathcal{O}\varepsilon\mathcal{O}}$ (DMRG) & $L$ & Index & $\lambda_{\mathcal{O}\varepsilon\mathcal{O}}$ (ED) & $\lambda_{\mathcal{O}\varepsilon\mathcal{O}}$ (DMRG) \\
\hline
0 & 0 ($\sigma_{(3)}$) & 1.4019 $(N=10)$ & 1.4097 $(N=18)$ & 4 & 2 & 1.8321 $(N=5)$ & -- \\ \hline
0 & 1 ($\partial \partial \sigma_{(3)}^{(0)}$) & 0.9629 $(N=10)$ & -- & 4 & 3 & 1.7899 $(N=5)$ & -- \\ \hline
1 & 0 ($\partial \sigma_{(3)}$) & 1.1141 $(N=10)$ & 1.1455 $(N=18)$ & 4 & 4 & 0.1674 $(N=5)$ & -- \\ \hline
2 & 0 ($\sigma_{(3)\mu\nu}$) & 0.8455 $(N=10)$ & 0.8996 $(N=18)$ & 4 & 5 & -0.1616 $(N=5)$ & -- \\ \hline
2 & 1 ($\partial \partial \sigma_{(3)}^{(2)}$) & 0.9065 $(N=10)$ & -- & 5 & 0 & 1.7514 $(N=5)$ & -- \\ \hline
3 & 0 ($\partial \partial \partial \sigma_{(3)}^{(3)}$) & 0.6484 $(N=10)$ & -- & 5 & 1 & 1.7506 $(N=5)$ & -- \\ \hline
4 & 0 & 0.8347 $(N=5)$ & -- & 5 & 2 & 0.1058 $(N=5)$ & -- \\ \hline
4 & 1 & 1.4946 $(N=5)$ & -- & 5 & 3 & -0.3275 $(N=5)$ & -- \\ \hline
\end{tabular}

==> OPE_Tables/OPE_Table_S4_+.tex <==
\begin{tabular}{|c|c|c|c||c|c|c|c|}
\hline
$L$ & Index & $\lambda_{\mathcal{O}\varepsilon\mathcal{O}}$ (ED) & $\lambda_{\mathcal{O}\varepsilon\mathcal{O}}$ (DMRG) & $L$ & Index & $\lambda_{\mathcal{O}\varepsilon\mathcal{O}}$ (ED) & $\lambda_{\mathcal{O}\varepsilon\mathcal{O}}$ (DMRG) \\
\hline
0 & 0 ($ t_{(4)}  $) & 1.7886 $(N=10)$ & 1.8049 $(N=18)$ & 2 & 1 ($\partial \partial t_{(4)}^{(2)}$) & -- & 1.3910 $(N=18)$ \\ \hline
1 & 0 ($\partial t_{(4)}^{(1)}$) & 1.5197 $(N=10)$ & 1.5682 $(N=18)$ & 3 & 0 & 0.8941 $(N=5)$ & -- \\ \hline
2 & 0 ($t_{(4)\mu\nu}$) & 1.0765 $(N=5)$ & 1.3565 $(N=18)$ & 4 & 0 & 0.8515 $(N=5)$ & -- \\ \hline
\end{tabular}

==> OPE_Tables/OPE_Table_S4_-.tex <==
\begin{tabular}{|c|c|c|c||c|c|c|c|}
\hline
$L$ & Index & $\lambda_{\mathcal{O}\varepsilon\mathcal{O}}$ (ED) & $\lambda_{\mathcal{O}\varepsilon\mathcal{O}}$ (DMRG) & $L$ & Index & $\lambda_{\mathcal{O}\varepsilon\mathcal{O}}$ (ED) & $\lambda_{\mathcal{O}\varepsilon\mathcal{O}}$ (DMRG) \\
\hline
0 & 0 & 2.1557 $(N=5)$ & -- & 3 & 0 & 1.9738 $(N=5)$ & -- \\ \hline
1 & 0 & 2.0522 $(N=10)$ & 2.0563 $(N=18)$ & 4 & 0 & 1.9506 $(N=5)$ & -- \\ \hline
2 & 0 & 2.0308 $(N=5)$ & -- &  & & &  \\ \hline
\end{tabular}

==> OPE_Tables/OPE_Table_S5_-.tex <==
\begin{tabular}{|c|c|c|c||c|c|c|c|}
\hline
$L$ & Index & $\lambda_{\mathcal{O}\varepsilon\mathcal{O}}$ (ED) & $\lambda_{\mathcal{O}\varepsilon\mathcal{O}}$ (DMRG) & $L$ & Index & $\lambda_{\mathcal{O}\varepsilon\mathcal{O}}$ (ED) & $\lambda_{\mathcal{O}\varepsilon\mathcal{O}}$ (DMRG) \\
\hline
0 & 0 ($\sigma_{(5)}$) & 2.1494 $(N=10)$ & 2.1794 $(N=18)$ &  & & &  \\ \hline
\end{tabular}

==> OPE_Tables/OPE_Table_S6_+.tex <==
\begin{tabular}{|c|c|c|c||c|c|c|c|}
\hline
$L$ & Index & $\lambda_{\mathcal{O}\varepsilon\mathcal{O}}$ (ED) & $\lambda_{\mathcal{O}\varepsilon\mathcal{O}}$ (DMRG) & $L$ & Index & $\lambda_{\mathcal{O}\varepsilon\mathcal{O}}$ (ED) & $\lambda_{\mathcal{O}\varepsilon\mathcal{O}}$ (DMRG) \\
\hline
0 & 0 & -- & 2.5347 $(N=18)$ &  & & &  \\ \hline
\end{tabular}
